A new selection method for high-dimensionial instrumental setting: application to the Growth Rate convergence hypothesis

This paper investigates the problem of selecting variables in regression-type models for an "instrumental" setting. Our study is motivated by empirically verifying the conditional convergence hypothesis used in the economical literature concerning the growth rate. To avoid unnecessary discussion about the choice and the pertinence of instrumental variables, we embed the model in a very high dimensional setting. We propose a selection procedure with no optimization step called LOLA, for Learning Out of Leaders with Adaptation. LOLA is an auto-driven algorithm with two thresholding steps. The consistency of the procedure is proved under sparsity conditions and simulations are conducted to illustrate the practical good performances of LOLA. The behavior of the algorithm is studied when instrumental variables are artificially added without a priori significant connection to the model. Using our algorithm, we provide a solution for modeling the link between the growth rate and the initial level of the gross domestic product and empirically prove the convergence hypothesis.

==> table.tex <==

\begin{figure}[h!]
 \begin{center}
 \begin{tabular}{ccc}
\includegraphics[height=4cm]{fig/corXYS10-dep0.eps} &
\includegraphics[height=4cm]{fig/corXYS10-dep1.eps} &
\includegraphics[height=4cm]{fig/corXYS50-dep0.eps}\\
Exp1&Exp2&Exp3
 \end{tabular}
 \end{center}
\caption{Empirical second moment between $Y$ and $X_1,\ldots,X_p$
for $p=2000$, $n=400$, the predictors $X'$s are gaussian. Exp1: The
predictors are independent, $S=10$. Exp2: The predictors are
dependent, $s=10$. Exp3: The predictors are independent, $S=50$. The
horizontal line is the auto-driven level $\hat t$.}
 \label{fig:1}
\end{figure}


\newpage

\begin{figure}[h!]
 \begin{center}
 \begin{tabular}{ccc}
\includegraphics[height=4cm]{fig/betaS10-dep0.eps} &
\includegraphics[height=4cm]{fig/betaS10-dep1.eps} &
\includegraphics[height=4cm]{fig/betaS50-dep0.eps}\\
Exp1&Exp2&Exp3
 \end{tabular}
 \end{center}
\caption{Estimators of the linear coefficients $\beta_\ell$ for
$\ell\in\cL$ for $p=2000$, $n=400$, the predictors $X'$s are
gaussian. Exp1: The predictors are independent, $S=10$. Exp2: The
predictors are dependent, $S=10$. Exp3: The predictors are
independent, $S=50$. The horizontal lines are the auto-driven levels
$\pm\,\hat s$.}
 \label{fig:2}
\end{figure}

\newpage

\begin{center}
\begin{table}[h!]
\begin{tabular}{rrrrr}
  \hline
 &  TN & TP & FN & FP \\
  \hline
Exp1& 1990.0 (1990) & 10.0 (10) & 0.0 (0) & 0.0 (0)\\
Exp2& 1989.9 (1990) & 9.2 (10)  & 0.8 (0) & 0.7 (0)\\
Exp3& 1948.8 (1950) & 36.1 (50) & 13.9 (0)& 1.2 (0) \\
  \hline
\end{tabular}
\caption{ Simulations performances for $K=100$ replications. The
true target value is given into brackets.\label{tableFNFP}}
  \end{table}

\end{center}

\newpage


\begin{figure} [h!]
 \begin{center}
 \begin{tabular}{ccc}
\includegraphics[width=5cm,height=3cm]{fig/betalolselectzoom.eps}&
\includegraphics[width=5cm,height=3cm]{fig/betaregselect.eps}&
\includegraphics[width=5cm,height=3cm] {fig/betastepselect.eps}\\
LOLA ($p=1213$) & OLS Student Selection($p=13$)& STEP ($p=13$)\\
\end{tabular}
\caption{Variables selection performances for Boston data, $K=100$
\label{BostonPerf}}
 \end{center}
 \end{figure}

 \newpage

 \vspace{0.5cm}
 {\footnotesize
\begin{center}
\begin{tabular}{cccccc}
\hline &$\widehat{\alpha_2}$&Confidence Interval &$N_0$& $R^2$&
p-value for $F$ test
\\\hline
Exp1&0.012  & [-0.038 , 0.062  ] & 1.000 & 0.005  & 0.673  \\
Exp2&0.017  & [-0.031 , 0.065 ] & 1.000 & 0.008  & 0.577   \\
Exp3&0.051  & [-0.002 , 0.104 ] & 1.000 & 0.045  & 0.139   \\
Exp4&0.058  & [\,0.006 , 0.111  ] & 1.000 & 0.060  & 0.085  \\\hline
\end{tabular}
 \end{center}
{TABLE 2: Estimation of the model $Y=\alpha_1+\alpha_2X+u$ for the
different periods of time. All the standard deviation values
normalized by $\sqrt{1000}$ are smaller than $10^{-3}$.}}

\newpage

\vspace{0.5cm}

\begin{center}{\footnotesize
\begin{tabular}{rccccc}
\hline &$\hat S$&$\widehat{\alpha_2}$&CI &$N_0$& p-value for $F$
test
\\\hline
Exp1&10.8 (0.1) & -0.245 (0.002) &[-0.358 (0.002), -0.132 (0.002)] & 0.011 (0.003) & 0.013 (0.001)\\
Exp2&10.9 (0.1) & -0.225 (0.002) &[-0.342 (0.002), -0.109 (0.002)] & 0.039 (0.006) & 0.025 (0.002)\\
Exp3&14.2 (0.1) & -0.227 (0.004) &[-0.429 (0.004), -0.025 (0.004)] & 0.452 (0.015) & 0.155 (0.005)\\
Exp4&14.6 (0.1) & -0.175 (0.004) &[-0.434 (0.005),  0.083 (0.004)] & 0.742 (0.014) & 0.255  (0.006)\\
&&&&\\
Exp1&6.3 (0.1) & -0.246 (0.002) &[-0.342 (0.002), -0.150 (0.001)] & 0.016 (0.004) & 0.007 (0.041)\\ %145   147   152   156   157
Exp2&6.3 (0.1) & -0.232 (0.002) &[-0.331 (0.002), -0.132 (0.001)] & 0.025 (0.005) & 0.011 (0.042)\\ %145   147   152   156   157
Exp3&8.4 (0.1) & -0.166 (0.003) &[-0.266 (0.003), -0.066 (0.002)] & 0.230 (0.013) & 0.004 (0.017)\\ %129   169   172   251   286   289   318   371   372
Exp4&8.4 (0.1) & -0.149 (0.003) &[-0.262 (0.003), -0.036 (0.002)] & 0.311 (0.014) & 0.009 (0.034)\\ %129   169   172   251   286   289   371   372& 0.310 (0.462) & 0.004 (0.022)\\
\hline
\end{tabular}

{TABLE 3: Estimation of $\alpha_2$ for determinants $Z$ selected via
Model 1 (above) and Model 2 (below). }}
\end{center}

 \newpage


 \begin{center}
 \begin{tabular}{cc}
\includegraphics[height=5cm,width=8cm]{fig/2histalpha6575ref60.eps} &
 \includegraphics[height=5cm,width=8cm]{fig/2histalpha7585ref70.eps}\\
{\footnotesize FIGURE 4. Exp1: 1965-75, $t_0=1960$, empirical
density of $\hat\alpha_2$}&{\footnotesize Exp3: 1975-85, $t_0=1970$,
empirical density of $\hat\alpha_2$}
 \end{tabular}
 \end{center}

\newpage

 \begin{center}
 \begin{tabular}{c}
\includegraphics[height=5cm,width=12cm]{fig/2selectcoeff6575ref60.eps}
\\
\includegraphics[height=5cm,width=12cm]{fig/2selectcoeff7585ref70.eps}
 \end{tabular}
 \end{center}
{\footnotesize{FIGURE 5. Selected variables for different periods
1965-1975, $t_0=$ 1960 (bottom) and 1975-1985, $t_0=$1970 (below).
Area 1: Education, Area 2: Population/Fertility, Area 3: Governement
Expendidures, Area 4: PPP deflators, Area 5: Political variables,
Area 6: Trade Policy and others.}}





\newpage

\begin{center}{\footnotesize
\begin{tabular}{rrcc|ccccc}
\hline &M&$\lambda$&$\hat S$&$\widehat{\alpha_2}$&CI
\\\hline
Exp1&BC&1.183&2& -0.016 &[-0.025, -0.004]\\
Exp1&BC&0.788&4& -0.041 &[-0.054, -0.029]\\
Exp1&BC&0.591&3& -0.044 &[-0.065, -0.034]\\
Exp1&BC&0.473&11&-0.051 &[-0.065, -0.032]\\
Exp1&M2&& 3  & -0.136 &[-0.212 , -0.060 ] \\ % 42    48    54
Exp2&M2&&3& -0.116  &[-0.191 , -0.040 ] \\ % 42    48    54
Exp3&M2&&11  & -0.351  &[-0.442 , -0.261 ]\\ %101   102   169   171   230   237   248   254   259   371   372
Exp4&M2&& 11  & -0.332  &[-0.443 , -0.221 ]\\ %101   102   169   171   230   237   248   254   259   371   372
\hline
\end{tabular}

{TABLE 4. Estimation of $\alpha_2$ for selection obtained via lasso
procedure and LOLA for Model2.}}
\end{center}

\newpage

\begin{center}
{\footnotesize
\begin{tabular}{cc|ccc}
\hline &$\hat S$&$\widehat{\alpha_2}$&CI &$N_0$
\\\hline
Exp1& 7.964  & -0.116  &[-0.146 , -0.085 ] & 0.001 \\
Exp2& 7.896  & -0.115  &[-0.144 , -0.085 ] & 0.000 \\
Exp3& 7.958  & -0.130  &[-0.165 , -0.096 ] & 0.002 \\
Exp4& 7.769  & -0.139  &[-0.172 , -0.106 ] & 0.000 \\
&&&&\\
Exp1& 8.772  & -0.085  &[-0.099 , -0.072 ] & 0.002 \\
Exp2& 8.736  & -0.083  &[-0.097 , -0.070 ] & 0.005  \\
Exp3& 8.766  & -0.096  &[-0.111 , -0.080 ] & 0.004 \\
Exp4& 8.773  & -0.094  &[-0.109 , -0.079 ] & 0.002 \\\hline
\end{tabular}}

{\footnotesize TABLE 5. Estimation of $\alpha_2$ for various periods
of time and for predictors $Z$ selected via Model1 (above) and
Model2 (below). All the standard deviation values normalized by
$\sqrt{1000}$ are smaller than $10^{-3}$. }
\end{center}
\newpage


 \begin{center}
 \begin{tabular}{cc}
\includegraphics[width=8cm,height=6cm]{fig/NP2histalpha6575ref60.eps} &
\includegraphics[width=8cm,height=6cm]{fig/NP2histalpha7585ref70.eps} \\
{\footnotesize FIGURE 6. Exp1: 1965-75, $t_0=1960$, empirical
density of $\hat\alpha_2$}&{\footnotesize Exp3: 1975-85, $t_0=1970$,
empirical density of $\hat\alpha_2$}
 \end{tabular}
 \end{center}
\newpage

\begin{center}{\footnotesize
\begin{tabular}{r|ccc|cccc}
\hline &$\hat S$&$\widehat{\alpha_2}$&CI &&$\hat
S$&$\widehat{\alpha_2}$&CI
\\\hline
Exp1& 8  & -0.120  &[-0.148 , -0.092 ] &        &8  & -0.086  &[-0.098 , -0.073 ] \\
Exp2& 8  & -0.116  &[-0.144 , -0.089 ]&         &8  & -0.083  &[-0.095 , -0.071 ] \\
Exp3& 8  & -0.133  &[-0.165 , -0.100 ] &        &9  & -0.100  &[-0.114 , -0.085 ] \\
Exp4&7  & -0.140  &[-0.172 , -0.108 ]  &        &9  & -0.093  &[-0.107 , -0.079 ]  \\
\hline
\end{tabular}

{TABLE 6. Estimation of $\alpha_2$ for both periods of time and for
determinants $Z$ selected via Model1 (left) and Model2 (right). }}
\end{center}

